Accretion disc winds imprint distinct signatures in the optical variability spectrum of black hole transients

Quantifying the variability, measured as the root mean square (rms), of accreting systems as a function of energy is a powerful tool for constraining the physical properties of these objects. Here, we present the first application of this method to optical spectra of low-mass X-ray binaries. We use high-time-resolution data of the black hole transient V404 Cygni, obtained with the \textit{Gran Telescopio Canarias} during its 2015 outburst. During this event, conspicuous wind-related features, such as P-Cygni profiles, were detected in the flux spectra. We find that rms spectra are rich in spectral features, although they are typically morphologically different from their flux counterparts. Specifically, we typically observe absorption components in correspondence to the presence of emission lines in the flux spectra. Similarly, when analysing segments with significant variability in the optical flux, P-Cygni line profiles appear inverted in the rms spectra (i.e., enhanced variability in the blue-shifted region, accompanied by a decrease in that associated with the red component). We discuss the possible origin of these features, which resemble those found in other objects, such as active galactic nuclei. Finally, we highlight the potential of this technique for future searches for wind-type outflows in accreting compact objects.

==> 0_RR.tex <==

We are thankful to the referee for his/her constructive and positive feedback. We are now submitting a new version of the manuscript, with changes highlighted in red. It follows a response (marked with **) to every referee's comment.

"This is a good paper, exploring a very new and interesting way to investigate accretion disc winds in X-ray binaries and other accreting systems via rms spectra. Overall it is well written, with topical and important scientific results. I recommend it for publication, but would like the authors to consider my comments, largely minor, listed below:"

**Thank you very much for the positive report.

INTRODUCTION

The authors state that there is no X-ray variability in the soft state -- this is not correct. The variability is much lower than the hard state, but there is still clearly some.

The final sentence of the introduction discusses ‘root-main-squared’ spectra, this should be ‘mean’.  

**Thanks for noticing this. Done.

RESULTS

The results in the paper are very interesting but could be presented a bit more clearly. The authors should consider that many interested readers will not be optical astronomers. Some thoughts:

Make ‘day-1’ etc ‘day 1’. I.e. remove the dash. In many studies authors set a ‘day zero’ and then discuss things which occurred before this in terms of negative day number. Hence the ‘day-1’ etc is confusing. 

**Done, we changed it both in the text and the figures

In 4.1 ‘blue part’ is not quantitatively defined in any way.

** We have rewritten the sentence to amend this problem.

I am not sure what the authors mean when that say that day-2 and day-6 are ‘the same datasets’.

** We apologise for the confusion, it just meant that we were analysing day 2 and day 6. We have modified the text to make it clear. 

Personally I think ‘block’ would be a good replacement for ‘chunk’ which is currently used. 

** Thanks for the suggestion. We agree that it does sound better. Done.

In the discussion of Fig 3, it is not very obvious that the P-Cygni profile becomes more prominent at low flux, as claimed (in contrast the rms changes are striking). 

**The referee is right. The sentence was not accurate. The P-Cyg profiles are equally conspicuous but the deepest blue-shifted absorptions (compared with the continuum, that is, in normalised spectra) are seen at low flux. We have modified the text to be more specific, leaving the reference to fig. 2 in MD2016, where a trailed spectrum is shown.  

I wonder, in a general sense, are ‘inverted P-Cygni’, ‘absorption’ etc - i.e. the language of flux spectra, appropriate for rms spectra? I genuinely do not know. Perhaps the existing literature in this field from X-rays, to which the authors refer, later, can shed some light on this. [ED:  In a sense, tthis is an abuse ofthe terminnology.  The resulting profile may *look* like an inverse P Cyg but that's just a statistical result, not a dynamical product; any such profile as a single realization (which yours isn't) is produced by a class of optically thick flows or velocity distributions.  You might have, for instance, more variation in the line center thanwings in some source but that doesn't mean you should use Lorentzian or Gausian as a descriptor.  The same here, you see a difference in variability depending on the radial velocity but that isn't what the photons are doing.  OK?.]

** We agree with the referee and the editor. To address this, we have revised several parts of the text. Specifically, we have introduced the term “inverted profile in rms,” which we believe resolves the issue while maintaining the term’s practicality. 

I think most/all of the figures could be better presented. Figs 1 and 3 in particular I had to keep switching between the text and the figure to understand what was being discussed. Additionally, will Fig 1 work for colour blind readers? Fig 2 panels should be individually labelled with the day and the line name, or something equally clear. The ‘yellow boxes’ are not really very easy to discern. Fig 2 caption should have a one-line summary of the main points that the figure shows.

** We thank the referee for the very useful suggestions. We tried to put Fig.1  and 3 close to each other (moving the Table 1 to another page). We have changed fig. 1 putting labels next to each curve, to help colour-blinded readers.  We have now increased the opacity of the boxes for more clarity. Finally an additional sentence has been added to the caption in Fig. 2.

Fig 3 the lines should be labelled, trying to cross match with the caption (which gives some wavelengths but not all) seems unnecessary.

** thanks for the advice. Done.

DISCUSSION

I am not sure I’d describe the 2015 V404 Cyg data as ‘textbook’ - doesn’t this usually imply canonical/standard behaviour, while we think V404 was quite extreme/odd?

**We have modified the sentence to be less ambiguous

I think ‘multi-faceted’ should replace ‘multi-factorial’, and the rest of this paragraph was not entirely clear to me, despite multiple re-reads. The authors state that the ‘relative abundance curve’ is steep for He III, which as I reader I assume is an experimentally/theoretically derived fact, but then the authors say it ‘might’ be flatter for He I or Balmer lines. I was left uncertain about what was known and what was not.
** We have re-written the paragraph. The main point is that theoretical predictions are also uncertain as they depend on many parameters.  Still, we feel that there might be some true in the provided explanation. Now, we acknowledge the purely exploratory nature of this discussion and stress the limitations in a more clear way. We have also modified the range of ionisation parameters quoted, which was too low for high densities according to the paper we refer (Kallman et al.). 

There is a ‘Munoz-Darias2016’ which looks like a LaTeX typo, maybe a missing \cite.
**Thanks for noticing. Done

The closing parts of the discussion in 5.1, discussing the important of joint flux and rms-spectral searches for wind signatures, was very good.
**Thanks. We do appreciate this very positive comment. 

In 5.2, in the sentence ‘From a theoretical…’ surely some mention of massive stars also, especially given the name of the feature?
** We agree with the referee. A more direct reference to massive stars was indeed mandatory. We have added it to the text.

